Waveforms for xG Non-stationary Channels

Waveform design for interference cancellation in next-generation wireless systems, which includes precoding and modulation, aims to achieve orthogonality among data signals/symbols across all Degrees of Freedom (DoF). Conventional methods struggle with non-stationary channel states due to high mobility, density, and time-varying multipath propagation. In this article, we review the HOGMT-Precoding and MEM modulations for non-stationary channels. We also discuss practical challenges and future directions.

==> background_icc.tex <==
\section{Background}
\label{sec:pre}
% \note{Zhibin: I removed some mentions of the LTV channel here and changed it to non-WSSUS check if this is correct.}

The wireless channel is typically expressed by a linear operator $H$, and the received signal $r(t)$ is given by $r(t){=}Hs(t)$, where $s(t)$ is the transmitted signal. The physics of the impact of $H$ on $s(t)$ is described using the delays and Doppler shifts in the multipath propagation~\cite{MATZ20111} given by \eqref{eq:H_delay_Doppler},
%
\begin{equation}
    r(t) = \sum\nolimits_{p=1}^P h_p s(t-\tau_p) e^{j2\pi \nu_p t}
    \label{eq:H_delay_Doppler}
\end{equation}
where $h_p$, $\tau_p$ and $\nu_p$ are the path attenuation factor, time delay and Doppler shift for path $p$, respectively. 
% The generalized form with respect to $\tau$ and $\nu$ is 
\eqref{eq:H_delay_Doppler} is expressed in terms of the overall delay $\tau$ and Doppler shift $\nu$ \cite{MATZ20111} in \eqref{eq:S_H}, 
% \eqref{eq:H_delay_Doppler} is rewritten in a general form %of $H$ 
% with respect to the overall delay $\tau$ and Doppler shift $\nu$ \cite{MATZ20111} in \eqref{eq:S_H}, 
%
\begin{align}
    % &r(t) = \iint S_H(\tau, \nu) s(t{-} \tau) e^{j2\pi \nu t} ~d\tau ~d\nu \label{eq:S_H} \\
    % & {=} \int L_H(t, f) S(f) e^{j2\pi tf} df; \enskip  L_H(t,f) {=} \iint S_H(\tau, \nu) e^{j2\pi (t\nu{-} f \tau)} d\tau d\nu \\
    % & {=} \int h(t, \tau) s(t{-} \tau) d\tau; \enskip h(t,\tau) {=} \int S_H(\tau, \nu) e^{j2\pi t \nu} d\nu \label{eq:h_relation}
    r(t) &= \iint S_H(\tau, \nu) s(t{-} \tau) e^{j2\pi \nu t} ~d\tau ~d\nu \label{eq:S_H} \\
    & = \int L_H(t, f) S(f) e^{j2\pi tf} ~df \\
    & = \int h(t, \tau) s(t{-} \tau) ~d\tau \label{eq:h_relation}
\end{align}
% where $S_H(\tau, \nu)$ is the \textit{(delay-Doppler) spreading function} of channel $H$, which describes the combined attenuation factor for all paths in the delay-Doppler domain. The time-frequency (TF) domain representation of $H$ is characterized by its \textit{TF transfer function}, $L_H(t,f)$, which is obtained by the 2-D Fourier transform of $S_H(\tau, \nu)$ as in \eqref{}. The time-varying response is $h(t,\tau) = \int S_H(\tau, \nu) e^{j2\pi t \nu} ~d\nu$.
where $S_H(\tau, \nu)$ is the \textit{(delay-Doppler) spreading function} of channel $H$, which describes the combined attenuation factor for all paths in the delay-Doppler domain. $S(f)$ is the Fourier transform of $s(t)$ and the time-frequency (TF) domain representation of $H$ is characterized by its \textit{TF transfer function}, $L_H(t,f)$, which is obtained by the 2-D Fourier transform of $S_H(\tau, \nu)$ as in \eqref{eq:TF_SH}. 
The time-varying impulse response $h(t,\tau)$ is obtained as the Inverse Fourier transform of $S_H(\tau, \nu)$ from the Doppler domain to the time domain as in  \eqref{eq:h_SH}.
\begin{align}
    L_H(t,f) &{=} \iint S_H(\tau, \nu) e^{j2\pi (t\nu{-} f \tau)} ~d\tau ~d\nu \label{eq:TF_SH}\\
    h(t,\tau) &{=} \int S_H(\tau, \nu) e^{j2\pi t \nu} ~d\nu \label{eq:h_SH}
\end{align}
% where $S_H(\tau, \nu)$ is the \textit{(delay-Doppler) spreading function} of channel $H$, which describes the combined attenuation factor for all paths in the delay-Doppler domain. $S(f)$ is the Fourier transform of $s(t)$ and the time-frequency (TF) domain representation of $H$ is characterized by its \textit{TF transfer function}, $L_H(t,f)$, which is obtained by the 2-D Fourier transform of $S_H(\tau, \nu)$ as $L_H(t,f) {=} \iint S_H(\tau, \nu) e^{j2\pi (t\nu{-} f \tau)} ~d\tau ~d\nu$. The time-varying response is $h(t,\tau) {=} \int S_H(\tau, \nu) e^{j2\pi t \nu} ~d\nu$.
% where $S_H(\tau, \nu)$ is the \textit{(delay-Doppler) spreading function} of channel $H$, which is the overall (all paths) attenuation factor at delay-Doppler domain. 
% \note{Do we need this: In this paper, we follow the LTV model in~\cite{MATZ20111}.}
% \ingreen{
% The time-varying response $h(t,\tau)$ of the channels is given by \eqref{eq:h_tau},
% \begin{equation}
% \label{eq:h_tau}
%     h(t,\tau) = \int S_H(\tau, \nu) e^{j2\pi t \nu} ~d\nu
% \end{equation}
% Maqsood: the $h(t,\tau$ in (21) is defined here.}
% The time-frequency (TF) domain representation of $H$ is characterized by its \textit{TF transfer function}, $L_H(t,f)$, which is obtained by the 2-D Fourier transform of $S_H(\tau, \nu)$ as in \eqref{eq:TH_L_H},
% \begin{align}
%     L_H(t,f) = \iint S_H(\tau, \nu) e^{j2\pi (t\nu{-} f \tau)} ~d\tau ~d\nu
%     \label{eq:TH_L_H}
% \end{align}
%
%
% For LTI channel TF transfer function is reduced to frequency response $L_H(t,f) {=} H(f)$. 
Figures \ref{fig:SH} and \ref{fig:LH} show the time-varying response and TF transfer function for an example of a time-varying channel. 
% \ingreen{Maqsood: I will show the $h(t,\tau)$ and $L_H(t,f)$ figures and they can both show NS. It's better to explain (6) and (7) by $h(t,\tau)$ instead of $S_H$.}
% \noindent
% \note{Is it needed:}
For stationary channels, the TF transfer function is a stationary process with $\mathbb{E}\{L_H(t, f) L_H^*(t',f')\} {=} R_H(t{-}t',f{-}f')$, and the spreading function is a white process (uncorrelated scattering), i.e., $\mathbb{E}\{S_H(\tau, \nu) S_H^*(\tau',\nu')\} {=} C_H(\tau,\nu) \delta (\tau{-} \tau') \delta(\nu{-} \nu')$, where $\delta(\cdot)$ is the Dirac delta function.
$C_H(\tau,\nu)$ and $R_H(t-t',f-f')$ are the \textit{scattering function} and \textit{TF correlation function}, respectively, which are related via 2-D Fourier transform, 
% as,
% \textbf{WSSUS channel:} 1) TF transfer function is a stationary process with $\mathbb{E}\{L_H(t, f) L_H^*(t',f')\} {=} R_H(t-t',f-f')$. 2) Spreading function is a white process (uncorrelated scattering), i.e., $\mathbb{E}\{S_H(\tau, \nu) S_H^*(\tau',\nu')\} {=} C_H(\tau,\nu) \delta (\tau{-} \tau') \delta(\nu{-} \nu')$ .
% $C_H(\tau,\nu)$ and $R_H(t-t',f-f')$ are \textit{scattering function} and \textit{TF correlation function}, respectively, which are related via 2-D Fourier transform
% \useshortskip
\begin{equation}
    C_H(\tau,\nu) = \iint R_H(\Delta t, \Delta f) e^{-j2\pi(\nu \Delta t -  \tau \Delta f)} ~d\Delta t ~d\Delta f
\end{equation}
% \noindent
% \textbf{Non-WSSUS channel:}
In contrast, for non-stationary channels, the TF transfer function is non-stationary process and the spreading function is a non-white process. %Since $C_H(\tau,\nu)$ is not defined for non-WSSUS channel, 
Therefore, a \textit{local scattering function} (LSF) $\mathcal{C}_H(t,f;\tau,\nu)$ \cite{MATZ20111} is defined to extend $C_H(\tau,\nu)$ to the non-stationary channels in \eqref{eq:LSF}. 
Similarly, the \textit{channel correlation function} (CCF) $\mathcal{R}(\Delta t, \Delta f;\Delta \tau, \Delta \nu)$ generalizes $R_H(\Delta t, \Delta f)$ to the non-stationary case in \eqref{eq:CCF}.
\begin{align}
\begin{split}
    &\mathcal{C}_H(t,f ; \tau,\nu)  \label{eq:LSF}\\
    & {=} {\iint} R_L(t, f; \Delta t, \Delta f) e^{-j2\pi(\nu \Delta t -  \tau \Delta f)} ~d\Delta t ~d\Delta f  \\
    & {=} \iint R_S(\tau, \nu; \Delta \tau, \Delta \nu) e^{-j2\pi(t \Delta \nu -  f \Delta \tau)} ~d\Delta \tau ~d\Delta \nu \\
\end{split}\\
\begin{split}
    &\mathcal{R}(\Delta t, \Delta f;\Delta \tau, \Delta \nu) \label{eq:CCF}\\
    & {=} \iint R_L(t, f; \Delta t, \Delta f) e^{-j2\pi(\Delta \nu  t -  \Delta \tau  f)} ~d t ~d f \\
    & {=} \iint R_S(\tau, \nu; \Delta \tau, \Delta \nu) e^{-j2\pi(\Delta t \nu -  \Delta f  \tau)} ~d \tau ~d \nu
\end{split}
\end{align}
where $R_L(t, f; \Delta t, \Delta f){=}\mathbb{E}\{L_H(t, f {+} \Delta f) L_H^*(t {-} \Delta t, f)\}$ and $R_S(\tau, \nu; \Delta \tau, \Delta \nu){=}\mathbb{E}\{S_H(\tau, \nu {+} \Delta \nu) S_H^*(\tau{-} \Delta \tau, \nu)\}$. 
For stationary channels, CCF reduces to TF correlation function $\mathcal{R}(\Delta t, \Delta f;\Delta \tau, \Delta \nu){=}R_H(\Delta t, \Delta f) \delta(\Delta t) \delta(\Delta f)$.
\textit{Due to space constraint, the complete proofs of Theorems and Lemmas are provided in an external document \cite{appendix_link}. 
% \ingreen{ they are defined by Matz' paper, not proved by us.}
}
% 
\vspace{-10pt}
\begin{figure}[h]
\begin{subfigure}{.24\textwidth}
  \centering
%   \includegraphics[trim={0 0 0 3cm},clip,width=1\linewidth]{figures/ht_tau_cropped.pdf}
\includegraphics[width=1\linewidth]{figures/ht_tau_cropped.pdf}
  \vspace{-20pt}
  \caption{Time-varying response $h(t,\tau)$}
  \label{fig:SH}
\end{subfigure}
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/L_H_cropped.pdf}
  \vspace{-20pt}
  \caption{TF transfer function $L_H(t,f)$}
  \label{fig:LH}
\end{subfigure}
\caption{Illustration of a non-stationary channel}
% \note{Is this time-varying or non-WSSUS? Change rotation of a) to match b)} 
  \vspace{-10pt}
\label{fig:toychannel}
\end{figure}
% \rood{Zhibin: Check whether eq.s (1)--(6) are directly used in the rest of the paper. If not, we need to cite and remove unless necessary somehow.} 

% \ingreen{Maqsood: In LTV channel, input relation of both WSSUS and non-WSSUS channel are the same ($h(t,\tau)$, $S_H$, $L_H$). We can only distinguish them by the statistics. That's why we need (6),(7) and other statistics to describes the non-WSSUS channel. They are not directly used but give us motivation to do unified characterization. Define unified characterization: all statistics/properties of any channel can be characterized by the same components (eigenvalues and eigenfunctions) decomposed by most general kernel $\mathcal{H}$}








\begin{comment}
Meanwhile, there is an inverse Fourier transformation from $\nu$ to $t$ in equation~\ref{eq:S_H}. Let $h(t,\tau) {=} \int S_H(\tau, \nu) e^{j2\pi \nu t} ~d\nu$, we have 

\begin{equation}
    r(t) = \int h(t,\tau) s(t{-} \tau) ~d\tau
\end{equation}
where $h(t,\tau)$ denotes time-varying impulse response. For NS channel, the correlation of time-varying response can be expressed as 

\begin{equation}
     R_h(t,\tau; \Delta t, \Delta \tau) \triangleq \mathbb{E}\{h(t,\tau+ \Delta \tau) h^*(t-\Delta t,\tau)\}
\end{equation}

In WSSUS channel case, $R_h(t,\tau; \Delta t, \Delta \tau) {=} R_h(\Delta t;\Delta \tau)$.  
\end{comment}


==> comment.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/data_flow.pdf}
    \caption{Data flow}
    \label{fig:Data_flow}
    \vspace{-10pt}
\end{figure*}

Figure~\ref{fig:Data_flow} shows the data flow of the space-time OFDM system. The kernel $k_H(u,t;u',t')$ has two explanations: 
\begin{enumerate}
    \item View from delay domain, the kernel can be seen as the time-varying delay response for MU case. The delay taps are non-stationary over time. The precoding aim to cancel ISI, IUI and ISI-IUI. 
    \item View from space domain, the kernel can be seen as time-varying space response with space delay. The space response are non-stationary over time. The precoding aim to cancel IUI and delayed IUI. 
\end{enumerate}

For the first explanation, it can also extend to space-time-frequency domain, where the kernel would be 6-D and the precoding can cancel ISI, IUI, ICI and ISI-ICI-IUI. For the second explanation, it can be seen as a MU precoding and can be combined with OFDM or OTFS.

\noindent
\textbf{Comparison with OTFS:} The OTFS delay-Doppler input-output relation can be expressed as continuous form
\begin{equation}
\label{eq:otfs_1}
    r(t,f) = \iint h_w(\tau, \nu) s(t - \tau, f - \nu) ~d\tau ~d\nu + v(t,f)
\end{equation}
where $v(\tau,\nu)$ is noise, and $h_w (\tau, \nu)$ is the convolution of delay-Doppler response $h_c(\tau, \nu)$ with window function $w(\tau,\nu)$ (Heisenberg transform):
\begin{equation}
\label{eq:otfs_2}
h_{w}(\tau, \nu)=\iint e^{-j 2 \pi \nu^{\prime} \tau^{\prime}} h_c\left(\tau^{\prime}, \nu^{\prime}\right) w\left(\nu-\nu^{\prime}, \tau-\tau^{\prime}\right) \mathrm{d} \tau^{\prime} \mathrm{d} \nu^{\prime}
\end{equation}

Notice $h_w(\tau, \nu)$ is the phase-shift correlation function of delay-Doppler response and window function for stationary case. \eqref{eq:otfs_1} is a composition of two Heisenberg transforms (Twisted convolution property), one corresponding to the modulation (window), and the other corresponding to the channel.

For kernel $K(u,t;u',t')$, the HOGMT precoding has different objective with OTFS and is not comparable but can combine with OTFS as the second explanation mentioned above. The HOGMT precoding is a general precoding method and can be applied to other kernels. To compare HOGMT precoding with OTFS but specify non-stationary channel, we define \textit{local spreading function} $h(t, f; \tau, \nu)$:

\begin{align}
\label{eq:deflsf}
    & h(t,f; \tau, \nu) \triangleq \mathbb{F}^2 \{ S_H(\tau, \nu + \Delta \nu) g^*(\tau - \Delta \tau, \nu) \} \nonumber \\
    & = \iint S_H(\tau, \nu + \Delta \nu) g^*(\tau - \Delta \tau, \nu) \nonumber \\
    & \times e^{j2\pi (t \Delta \nu - f \Delta \tau)} ~d\Delta \tau ~d\Delta \nu
\end{align}
which denotes delay-Doppler complex attenuation at TF location $(t,f)$. $g(\tau, \nu)$ is the window function with $\iint ||g(\tau,\nu)||^2 ~d\tau ~d\nu {=} 1$. 

The multi-carrier input-output relation for non-stationary channel can be written as 
\begin{equation}
\label{eq:h}
    r(t,f) = \iint h(t,f; \tau, \nu) s(t - \tau, f - \nu) ~d\tau ~d\nu + v(t,f)
\end{equation}

Notice~\eqref{eq:deflsf} and~\eqref{eq:h} has the similar form with~\eqref{eq:otfs_1} and~\eqref{eq:otfs_2}, respectively, but for non-stationary case. OTFS reduce the interference by designing symbols which experience minimal cross. It transmit symbols through delay-Doppler domain where existing less interference than time-frequency domain. However, equalizer is still required to cancel the OTFS intersymbol interference. While HOGMT precoding decompose the channel kernel to jointly orthogonal eigenfunctions (dual-flat fading sub-channels) and design waveform to cancel total interference of the channel. 

\setlength{\textfloatsep}{0.1cm}
\setlength{\tabcolsep}{0.2em}
\begin{table}[h]
\caption{Comparison between OTFS and HOGMT-Precoding}
\renewcommand*{\arraystretch}{1.2}
\centering
\begin{tabular}{|l|l|l|}
\hline
Techniques & OTFS & HOGMT-Precoding \\ \hline
Types     &  Modulation & Precoding\\ \hline
CSI & Perfect CSI at Rx & Perfect CSI at TX             \\ \hline
Channel   &  Staionary & Non-Stationary    \\ \hline
Interference-free & No & Yes \\ \hline
Extension to MU-MIMO &  Additional Equalizer  &  Yes  \\ \hline
\end{tabular}
\label{tab:cha}
\vspace{-10pt}
\end{table}

Overall, OTFS can make general channels "generate" less interference. HOGMT-Precoding is specific to each channel and can cancel existing interference of that channel. 

==> conclusion_icc22.tex <==
\section{Conclusion}
\label{sec:conclusion}

% \note{Rewrite:
% \ingreen{This paper answer Marts' open problem: How can non-WSSUS be decomposed into flat fading channels. By GMT, the channel is decomposed into \textbf{dual eigen flat fading subchannels}. When we transmit one eigenfunctions set with coefficients, because of eigen properties, we actually transfer another eigenfunctions set with the coefficients, which atomic reconstruct data signal.}
In this work, we derived a high-order generalized version of Mercer's Theorem to decompose the general non-stationary channel kernel into 2-dimensional jointly orthogonal flat fading sub-channels (eigenfunctions).
Through theoretical analysis and simulations, we draw three firm conclusions for non-stationary channels: 1) The 2-dimensional eigenfunctions are sufficient to completely derive the second-order statistics of the non-stationary channel and consequently leads to an %accurate and 
unified characterization of any wireless channel, 2) precoding by combining these eigenfunctions with optimally derived coefficients %leads to 
mitigates the spatio-temporal interference, %in non-stationary channels
% mitigates the independent and joint spatio-temporal interference achieving \ingreen{near AWGN BER}
and 3) the precoded symbols when propagated over the non-stationary channel directly reconstruct the data symbols at the receiver when combined with calculated coefficients, consequently alleviating the need for complex complementary decoding at the receiver.
Therefore, the encouraging results from this work will form the core of robust and unifed characterization and highly reliable communication over nonstationary channels, supporting emerging application.
% We propose the generalized Mercer's theorem to decompose the channel kernel into different eigenfunctions. Non-WSSUS channel properties are unifiedly characterized by the decomposed eigenvalues and eigenfunctions. 
% 

% We also studied the precoding technique with eigenfunctions and shows that because of the orthonormal property of eigenfunctions, we can propagate eigenfunctions of channel kernel 
% % \ingreen{not eigenfunctions of channel kernel. eigenfunctions of channel kernel also can have the same dimension by KLT. should be eigenfunctions decomposed by GMT} 
% to achieve the orthornomal projections, which can automatic construct data signals with certain coefficients. 
% }

\section{ACKNOWLEDGEMENT}
This work is funded by the Air Force Research Laboratory Visiting Faculty Research Program (SA10032021050367), Rome, New York, USA.

\begin{comment}
In this paper, the local spreading function is proposed to specify the non-WSSUS channel, which can be decomposed into the time-frequency eigenfunction and delay-Doppler eigenfunction by the proposed novel decomposition method. The statistics is well characterized by the decomposed eigenfunctions and eigenvalues.  

We also studied the precoding technique for non-WSSUS channel and shows that because of the orthonormal property of eigenfunctions, we can propagate eigenfunctions of non-WSSUS channel kernel in delay-Doppler domain to achieve the orthornomal projections in time-frequency domain. With the novel decomposition method, the non-WSSUS channel precoding can achieve interference-free performance.

In the future work, we will investigate more precoding strategies based on non-WSSUS channel decomposition and study the implementation for MU-MIMO non-WSUSS case. 
\end{comment}


\begin{comment}
In this paper, we studied the interpretation of neural network based receivers for single and multiple antenna systems. 
Through rigorous theoretical and empirical analysis we show that a feed-forward deep NN-based receiver with the MSE loss function is equivalent to the optimal classical MAP receiver, under sufficiently rich training. 
We show that under finite training, the expected error is distributed as a Gaussian, and derive tight upper bounds on the BER of the NN-based receivers. %, under finite training samples. 
Extensive practical simulations have corroborated that the BER of such NN-based receivers are within the derived theoretical bounds, and cannot outperform optimal classical receivers when a rigorous mathematical channel model is available. 
% These results show that a single neural network can replace the classical receiver, and learns a computationally tractable algorithm to decode the received signal regardless of the channel condition. 
Moreover, we empirically derive the model of the NN-based receiver for which the error rate is minimum for a given data-set.
The guarantees on the achievable error rate of NN-based receivers is a necessary step towards ensuring wide-spread adoption of NN-based transceivers in xG systems. 
% Furthermore, under incomplete training the BER can be minimized by optimizing the hyper parameters such as the depth and width of the NN-based receiver, which is currently being investigated. 

% However, the DL estimator is sensitive to the quality of training data and its performance would significantly degrade if the data in real environments distributes broader than the training data. 
% The benefits of the DL estimator have to weigh against its costs when applied to the channel estimation in real wireless communication systems. We should strike a balance between DL based channel estimation and traditional channel estimation.


%\note{add more to the conclusion}
% In this paper, we studied the opportunities and limitations of NN-based transceivers over classical approaches for wireless communications.
% Through theoretical proofs, simulation and analysis we draw the following conclusions: 
% 1) the equivalence of NN-based and classical transceivers under known and stationary channels, 
% 2) NN-based transceivers outperform classical transceivers under unknown channel distributions and non-stationary statistics.
% 3) the inverse design of NN-based transceivers achieve guaranteed BER performance,
% Therefore, NN-based transceiver design is only useful in wireless communications, if properly designed and under certain channel conditions. 
\end{comment}













































